The Best of Both Worlds: On the Dilemma of Out-of-distribution Detection

Out-of-distribution (OOD) detection is essential for model trustworthiness which aims to sensitively identify semantic OOD samples and robustly generalize for covariate-shifted OOD samples. However, we discover that the superior OOD detection performance of state-of-the-art methods is achieved by secretly sacrificing the OOD generalization ability. Specifically, the classification accuracy of these models could deteriorate dramatically when they encounter even minor noise. This phenomenon contradicts the goal of model trustworthiness and severely restricts their applicability in real-world scenarios. What is the hidden reason behind such a limitation? In this work, we theoretically demystify the ``\textit{sensitive-robust}'' dilemma that lies in many existing OOD detection methods. Consequently, a theory-inspired algorithm is induced to overcome such a dilemma. By decoupling the uncertainty learning objective from a Bayesian perspective, the conflict between OOD detection and OOD generalization is naturally harmonized and a dual-optimal performance could be expected. Empirical studies show that our method achieves superior performance on standard benchmarks. To our best knowledge, this work is the first principled OOD detection method that achieves state-of-the-art OOD detection performance without compromising OOD generalization ability. Our code is available at \href{https://github.com/QingyangZhang/DUL}{https://github.com/QingyangZhang/DUL}.

==> tables/tab-cifar10.tex <==
\begin{table}[!htbp]
\centering
\caption{Comprehensive comparison involving 15 different types of corruption from commonly-used domain adaption benchmark [52]. Substantial ($\geq0.5$) \textcolor{mycolor4}{improvement} and \textcolor{mycolor3}{degradation} compared to the baseline MSP [6] are highlighted in \textcolor{mycolor4}{blue} or \textcolor{mycolor3}{red} respectively. DUL is the only method that achieves SOTA OOD detection performance without sacrificing generalization i.e., the value of the entire row is almost black or blue. The \textbf{best} or \underline{second best} results are highlighted in bold or underlined. MD is the shorthand of Mahalanobis.}
\vskip 4pt
\label{tab:ood generalization cifar10-C}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{0.75mm}
\begin{tabular}{c|c|c|ccccccccccccccc|c|cc}
\toprule
 \multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} & \multicolumn{16}{c}{OOD generalization (Error rate $\downarrow$)} & \multicolumn{2}{c}{OOD detection} \\  
  Method &$\mathcal{P}^{\rm ID}_{\rm train}$  &$\mathcal{P}^{\rm SEM}_{\rm train}$ &  Gauss. & Shot & Impul. & Defoc. & Glass & Motion & Zoom & Snow & Frost & Fog & Brit. & Contr. &Elast. &Pixel &JPEG &Avg. &FPR$\downarrow$ &AUC$\uparrow$\\
\midrule
MSP &\multirow{18}{*}{\rotatebox{90}{CIFAR-10}} &\multirow{4}{*}{\rotatebox{90}{None}} & 77.0 & 67.7 & 74.5 & 36.1 & 78.5 & 40.7 & 41.4 & 40.5 & 46.7 & 31.4 & 22.6 & 40.3 & 35.3 & 42.8 & 44.9 & 48.0 &42.0 &89.3\\EBM  & & & 77.0 & 67.7 & 74.5 & 36.1 & 78.5 & 40.7 & 41.4 & 40.5 & 46.7 & 31.4 & 22.6 & 40.3 & 35.3 & 42.8 & 44.9 & 48.0&32.5 &89.3\\Maxlogits & & &77.0 & 67.7 & 74.5 & 36.1 & 78.5 & 40.7 & 41.4 & 40.5 & 46.7 & 31.4 & 22.6 & 40.3 & 35.3 & 42.8 & 44.9 & 48.0 &32.9 &89.3 \\ MD & & & 77.0 & 67.7 & 74.5 & 36.1 & 78.5 & 40.7 & 41.4 & 40.5 & 46.7 & 31.4 & 22.6 & 40.3 & 35.3 & 42.8 & 44.9 & 48.0 &32.5 &93.9 \\
\cline{1-1} \cline{3-21} Entropy& &\multirow{7}{*}{\rotatebox{90}{ImageNet-RC}} &\textcolor{mycolor3}{81.7} & \textcolor{mycolor3}{72.9} & \textcolor{mycolor3}{87.0} & \textcolor{mycolor3}{38.2} & \textcolor{mycolor3}{88.9} & \textcolor{mycolor3}{42.2} & \textcolor{mycolor3}{44.6} & \textcolor{mycolor3}{45.5} & \textcolor{mycolor3}{53.9} & \textcolor{mycolor3}{33.1} & \textcolor{mycolor3}{24.4} & \textcolor{mycolor4}{39.8} & \textcolor{mycolor3}{37.2} & \textcolor{mycolor3}{47.6} & \textcolor{mycolor3}{48.8} & \textcolor{mycolor3}{52.4} &\textcolor{mycolor4}{6.6} &\textcolor{mycolor4}{\underline{98.7}}\\EBM (FT) & & &\textcolor{mycolor3}{82.3} & \textcolor{mycolor3}{73.5} & \textcolor{mycolor3}{90.6} & \textcolor{mycolor3}{39.2} & \textcolor{mycolor3}{90.7} & \textcolor{mycolor3}{41.4} & \textcolor{mycolor3}{44.4} & \textcolor{mycolor3}{47.3} & \textcolor{mycolor3}{54.9} & \textcolor{mycolor3}{34.3} & \textcolor{mycolor3}{24.7} & \textcolor{mycolor4}{\textbf{39.2}} & \textcolor{mycolor3}{37.7} & \textcolor{mycolor3}{51.5} & \textcolor{mycolor3}{49.3} & \textcolor{mycolor3}{53.4} &\textcolor{mycolor4}{\underline{3.6}} &\textcolor{mycolor4}{98.4}\\DPN & & &\textcolor{mycolor3}{77.6} & \textcolor{mycolor3}{68.6} & \textcolor{mycolor3}{83.6} & \textcolor{mycolor3}{39.7} & \textcolor{mycolor3}{86.8} & \textcolor{mycolor3}{43.3} & \textcolor{mycolor3}{44.9} & \textcolor{mycolor3}{47.0} & \textcolor{mycolor3}{53.7} & \textcolor{mycolor3}{36.4} & \textcolor{mycolor3}{26.1} & \textcolor{mycolor3}{43.5} & \textcolor{mycolor3}{37.6} & \textcolor{mycolor3}{47.5} & \textbf{44.5} & \textcolor{mycolor3}{52.0} &\textcolor{mycolor4}{4.3} &\textcolor{mycolor4}{98.5}\\ POEM & & & \textcolor{mycolor3}{83.7} & \textcolor{mycolor3}{76.6} & \textcolor{mycolor3}{88.0} & \textcolor{mycolor3}{44.1} & \textcolor{mycolor3}{90.1} & \textcolor{mycolor3}{44.3} & \textcolor{mycolor3}{46.4} & \textcolor{mycolor3}{52.8} & \textcolor{mycolor3}{60.8} & \textcolor{mycolor3}{39.5} & \textcolor{mycolor3}{28.9} & \textcolor{mycolor3}{43.4} & \textcolor{mycolor3}{42.5} & \textcolor{mycolor3}{56.1} & \textcolor{mycolor3}{54.5} & \textcolor{mycolor3}{56.8} &\textcolor{mycolor4}{\textbf{3.3}} &\textcolor{mycolor4}{\textbf{99.0}}\\WOODS & & &\textcolor{mycolor3}{77.5} & \textcolor{mycolor3}{68.5} & \textcolor{mycolor3}{77.5} & 36.4 & \textcolor{mycolor3}{80.6} & \underline{40.9} & \textcolor{mycolor3}{41.9} & \textcolor{mycolor3}{41.3} & 47.1 & \underline{31.4} & \textcolor{mycolor3}{23.3} & \textcolor{mycolor4}{\underline{39.7}} & \textcolor{mycolor3}{36.2} & \underline{42.9} & \textcolor{mycolor3}{46.2} & \textcolor{mycolor3}{48.8} &\textcolor{mycolor4}{7.1} &\textcolor{mycolor4}{98.5}\\SCONE& & & \textcolor{mycolor4}{\textbf{76.4}} & \textbf{67.3} & \textcolor{mycolor3}{\underline{75.3}} & \underline{36.2} & \textcolor{mycolor4}{\textbf{77.0}} & \underline{40.9} & \underline{41.6} & \underline{40.2} & \textcolor{mycolor4}{\textbf{45.5}} & \underline{31.4} & \textcolor{mycolor3}{\underline{23.1}} & 40.1 & \textcolor{mycolor3}{\underline{35.9}} & \textbf{42.4} & \textcolor{mycolor3}{45.4} & \underline{47.9} &\textcolor{mycolor4}{7.0} &\textcolor{mycolor4}{98.5}\\DUL (Ours) & & &\cellcolor{gray!20}\underline{77.2} & \cellcolor{gray!20}\underline{68.0} & \cellcolor{gray!20}\textcolor{mycolor3}{\textbf{75.1}} & \cellcolor{gray!20}\textbf{35.8} & \cellcolor{gray!20}\underline{78.5} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{39.7}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{40.6}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{39.8}} & \cellcolor{gray!20}\textcolor{mycolor4}{\underline{46.1}} & \cellcolor{gray!20}\textbf{31.0} & \cellcolor{gray!20}\textbf{22.4} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{39.2}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{34.8}} & \cellcolor{gray!20}43.0 & \cellcolor{gray!20}\underline{44.6} & \cellcolor{gray!20}\textbf{47.7} &\cellcolor{gray!20}\textcolor{mycolor4}{5.9} &\cellcolor{gray!20}\textcolor{mycolor4}{98.5}\\
\cline{1-1} \cline{3-21} Entropy & &\multirow{7}{*}{\rotatebox{90}{TIN-597}} & \textcolor{mycolor3}{83.3} & \textcolor{mycolor3}{75.4} & \textcolor{mycolor3}{79.8} & \textcolor{mycolor3}{38.0} & \textcolor{mycolor3}{82.7} & \textcolor{mycolor3}{\underline{42.2}} & \textcolor{mycolor3}{44.2} & \textcolor{mycolor3}{44.5} & \textcolor{mycolor3}{53.4} & \textcolor{mycolor3}{32.8} & \textcolor{mycolor3}{\underline{23.7}} & \textcolor{mycolor4}{\textbf{38.0}} & \textcolor{mycolor3}{37.9} & \textcolor{mycolor3}{44.6} & \textcolor{mycolor3}{62.9} & \textcolor{mycolor3}{52.2} &\textcolor{mycolor4}{11.6} &\textcolor{mycolor4}{97.9}\\EBM (FT) & & &\textcolor{mycolor3}{81.2} & \textcolor{mycolor3}{72.8} & \textcolor{mycolor3}{78.1} & \textcolor{mycolor3}{\underline{37.6}} & \textcolor{mycolor3}{80.0} & \textcolor{mycolor3}{42.9} & \textcolor{mycolor3}{43.6} & \textcolor{mycolor3}{43.7} & \textcolor{mycolor3}{51.1} & \textcolor{mycolor3}{33.5} & \textcolor{mycolor3}{23.9} & 40.2 & \textcolor{mycolor3}{38.1} & \textcolor{mycolor3}{45.1} & \textcolor{mycolor3}{73.3} & \textcolor{mycolor3}{52.3}&\textcolor{mycolor4}{19.4} &\textcolor{mycolor3}{87.5}\\DPN & & &\textcolor{mycolor3}{81.8} & \textcolor{mycolor3}{72.9} & \textcolor{mycolor3}{79.1} & \textcolor{mycolor3}{39.6} & \textcolor{mycolor3}{81.3} & \textcolor{mycolor3}{44.9} & \textcolor{mycolor3}{46.2} & \textcolor{mycolor3}{45.4} & \textcolor{mycolor3}{52.4} & \textcolor{mycolor3}{34.3} & \textcolor{mycolor3}{25.6} & \textcolor{mycolor3}{40.9} & \textcolor{mycolor3}{39.2} & \textcolor{mycolor3}{47.7} & \textcolor{mycolor3}{76.4} & \textcolor{mycolor3}{53.8}&\textcolor{mycolor4}{17.3} &\textcolor{mycolor4}{94.9}\\POEM & & &\textcolor{mycolor3}{\underline{78.9}} & \textcolor{mycolor3}{\underline{70.3}} & \underline{74.7} & \textcolor{mycolor3}{38.6} & \textcolor{mycolor4}{\textbf{78.0}} & \textcolor{mycolor3}{43.4} & \textcolor{mycolor3}{44.3} & \textcolor{mycolor3}{43.0} & \textcolor{mycolor3}{50.2} & \textcolor{mycolor3}{34.6} & \textcolor{mycolor3}{25.4} & \textcolor{mycolor3}{43.1} & \textcolor{mycolor3}{\underline{37.3}} & \textcolor{mycolor3}{45.4} & \textcolor{mycolor3}{81.6} & \textcolor{mycolor3}{52.6} &\textcolor{mycolor4}{34.3} &\textcolor{mycolor3}{86.8}\\WOODS & & & \textcolor{mycolor3}{81.1} & \textcolor{mycolor3}{72.4} & \textcolor{mycolor3}{76.5} & \textcolor{mycolor3}{38.6} & \textcolor{mycolor3}{79.0} & \textcolor{mycolor3}{43.2} & \textcolor{mycolor3}{44.6} & \textcolor{mycolor3}{\underline{42.4}} & \textcolor{mycolor3}{\underline{49.2}} & \textcolor{mycolor3}{33.0} & \textcolor{mycolor3}{24.3} & 40.2 & \textcolor{mycolor3}{39.0} & \textcolor{mycolor4}{\textbf{41.2}} & \textcolor{mycolor3}{\underline{47.8}} & \textcolor{mycolor3}{50.2} &\textcolor{mycolor4}{\underline{7.6}} &\textcolor{mycolor4}{\textbf{98.3}}\\SCONE & & & \textcolor{mycolor3}{80.9} & \textcolor{mycolor3}{72.3} & \textcolor{mycolor3}{77.2} & \textcolor{mycolor3}{37.9} & 78.7 & \textcolor{mycolor3}{42.4} & \textcolor{mycolor3}{\underline{43.4}} & \textcolor{mycolor3}{42.8} & \textcolor{mycolor3}{49.5} & \textcolor{mycolor3}{\underline{32.2}} & \textcolor{mycolor3}{24.0} & \textcolor{mycolor4}{\underline{39.3}} & \textcolor{mycolor3}{38.0} & \textcolor{mycolor4}{\underline{41.8}} & \textcolor{mycolor3}{48.3} & \textcolor{mycolor3}{\underline{50.0}} &\textcolor{mycolor4}{8.0} &\textcolor{mycolor4}{\underline{98.2}}\\DUL (Ours)& & &\cellcolor{gray!20}\textbf{77.0} & \cellcolor{gray!20}\textbf{67.7} & \cellcolor{gray!20}\textbf{74.2} & \cellcolor{gray!20}\textbf{36.2} & \cellcolor{gray!20}\underline{78.4} & \cellcolor{gray!20}\textbf{40.8} & \cellcolor{gray!20}\textbf{41.3} & \cellcolor{gray!20}\textbf{40.2} & \cellcolor{gray!20}\textbf{46.3} & \cellcolor{gray!20}\textbf{31.4} & \cellcolor{gray!20}\textbf{22.9} & \cellcolor{gray!20}\textcolor{mycolor3}{40.8} & \cellcolor{gray!20}\textbf{35.3} & \cellcolor{gray!20}42.7 & \cellcolor{gray!20}\textbf{45.1} & \cellcolor{gray!20}\textbf{48.0}&\cellcolor{gray!20}\textcolor{mycolor4}{\textbf{6.9}} &\cellcolor{gray!20}\textcolor{mycolor4}{\underline{98.2}}\\
\midrule \midrule

MSP &\multirow{9}{*}{\rotatebox{90}{ImageNet-200}} &\multirow{3}{*}{\rotatebox{90}{None}} & 52.2 & 70.7 & 71.5 & 56.0  &55.5  & 52.6 & 54.1 & 67.3 & 67.0 & 63.5 &56.5& 53.3&46.3 &50.3&51.9&57.9 &58.2 &82.3\\EBM  & & & 52.2 & 70.7 & 71.5 & 56.0  &55.5  & 52.6 & 54.1 & 67.3 & 67.0 & 63.5 &56.5& 53.3&46.3 &50.3&51.9&57.9&32.5 &89.3\\Maxlogits & & &52.2 & 70.7 & 71.5 & 56.0  &55.5  & 52.6 & 54.1 & 67.3 & 67.0 & 63.5 &56.5& 53.3&46.3 &50.3&51.9&57.9 &51.9 &88.2 \\
\cline{1-1} \cline{3-21} Entropy& &\multirow{6}{*}{\rotatebox{90}{ImageNet-800}} & \textcolor{mycolor4}{\underline{51.3}}&\textcolor{mycolor3}{71.2}&71.7&\textcolor{mycolor4}{\textbf{54.4}}&\textcolor{mycolor4}{\underline{54.6}}&\textcolor{mycolor4}{\underline{51.8}}&\textcolor{mycolor4}{53.2}&\textcolor{mycolor4}{66.9}&\textcolor{mycolor4}{66.2}&\textcolor{mycolor4}{62.7}&\textcolor{mycolor4}{55.8}&\textcolor{mycolor4}{\textbf{51.4}}&\textcolor{mycolor4}{\textbf{45.1}}&\textcolor{mycolor4}{\underline{49.7}}&\textcolor{mycolor4}{\underline{51.1}}&\textcolor{mycolor4}{57.1} &\textcolor{mycolor4}{53.6} &\textcolor{mycolor4}{\underline{89.1}}\\EBM (FT) & & &\textcolor{mycolor3}{52.9}&\textcolor{mycolor3}{72.2}&\textcolor{mycolor3}{72.8}&56.0&\textcolor{mycolor3}{56.2}&\textcolor{mycolor3}{53.5}&54.1&\textcolor{mycolor3}{67.8}&67.4&\textcolor{mycolor3}{64.0}&\textcolor{mycolor3}{57.0}&\textcolor{mycolor4}{\underline{52.2}}&46.5&\textcolor{mycolor3}{51.4}&\textcolor{mycolor3}{52.9}&\textcolor{mycolor3}{58.5}&\textcolor{mycolor3}{59.7} &\textcolor{mycolor4}{87.5}\\DPN & & & 51.9 & \textcolor{mycolor4}{\underline{69.2}} & \textcolor{mycolor4}{\textbf{69.6}} & \textcolor{mycolor3}{56.5} & 55.6 & 52.4 & \textcolor{mycolor4}{53.1} & \textcolor{mycolor4}{\textbf{65.5}} & \textcolor{mycolor4}{\textbf{65.0}} & \textcolor{mycolor4}{\textbf{62.2}} & \textcolor{mycolor4}{\textbf{55.5}} & \textcolor{mycolor3}{54.5} & 46.0 & \textcolor{mycolor4}{\underline{49.7}} & \textcolor{mycolor4}{51.4} & \textcolor{mycolor4}{57.2} &\textcolor{mycolor3}{63.8} &87.2\\WOODS & & &\textcolor{mycolor4}{51.4} & \textcolor{mycolor4}{69.4} & \textcolor{mycolor4}{\underline{70.0}} & \textcolor{mycolor4}{55.2} & \textcolor{mycolor4}{54.8} & \textcolor{mycolor4}{51.9} & \textcolor{mycolor4}{\underline{52.9}} & \textcolor{mycolor4}{\underline{66.2}} & \textcolor{mycolor4}{66.0} & \textcolor{mycolor4}{\underline{62.5}} & \textcolor{mycolor4}{\underline{55.6}} & \textcolor{mycolor4}{52.6} & \textcolor{mycolor4}{45.6} & \textcolor{mycolor4}{\underline{49.7}} & \textcolor{mycolor4}{51.3} & \textcolor{mycolor4}{\underline{57.0}} &\textcolor{mycolor4}{\underline{51.7}} &\textcolor{mycolor4}{88.3}\\SCONE& & &\textcolor{mycolor4}{51.6} & \textcolor{mycolor4}{69.4} & \textcolor{mycolor4}{\underline{70.0}} & \textcolor{mycolor4}{55.4} & \textcolor{mycolor4}{55.0} & \textcolor{mycolor4}{52.1} & \textcolor{mycolor4}{53.1} & \textcolor{mycolor4}{66.3} & \textcolor{mycolor4}{66.0} & \textcolor{mycolor4}{62.6} & \textcolor{mycolor4}{55.7} & 53.0 & \textcolor{mycolor4}{45.8} & 49.9 & \textcolor{mycolor4}{51.4} & \textcolor{mycolor4}{57.1}&\textcolor{mycolor4}{52.5} &\textcolor{mycolor4}{88.2}\\DUL (Ours) & & &\cellcolor{gray!20}\textcolor{mycolor4}{\textbf{51.0}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{69.1}} & \cellcolor{gray!20}\textcolor{mycolor4}{70.5} & \cellcolor{gray!20}\textcolor{mycolor4}{\underline{55.1}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{54.5}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{51.5}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{52.4}} & \cellcolor{gray!20}\textcolor{mycolor4}{\underline{66.2}} & \cellcolor{gray!20}\textcolor{mycolor4}{\underline{65.9}} & \cellcolor{gray!20}\textcolor{mycolor4}{62.6} & \cellcolor{gray!20}\textcolor{mycolor4}{55.7} & \cellcolor{gray!20}53.0 & \cellcolor{gray!20}\textcolor{mycolor4}{\underline{45.4}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{49.4}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{50.9}} & \cellcolor{gray!20}\textcolor{mycolor4}{\textbf{56.9}} &\cellcolor{gray!20}\textcolor{mycolor4}{\textbf{49.1}} &\cellcolor{gray!20}\textcolor{mycolor4}{\textbf{89.3}}\\
\bottomrule
\end{tabular}
}
\vskip -0.0in
\end{table}


==> tables/table2.tex <==
\begin{table*}[htbp]
\begin{center}
% \begin{spacing}{1.35}   
%\small
\caption{OOD detection and generalization performance comparison on ImageNet. Substantial \textcolor{mycolor4}{improvement} and \textcolor{mycolor3}{degradation} ($\geq 0.5$) compared to baseline (MSP) are highlighted in blue or red respectively. The \textbf{best} and \underline{second best} results are in bold or underlined. Similar with CIFAR experiments, our method establishes strong OOD detection performance (always the best or second best) without degraded generalization ability, i.e., the entire row is either blue or black. Full results with diverse types of corruption are in the Appendix~\ref{appendix:more-results}.}
\vskip -0.03in
\label{tab:imagenet}
\center
\resizebox{1.0\textwidth}{!}{
\setlength{\tabcolsep}{3.9mm}
\begin{tabular}{cc|cc|ccc}
\toprule \multirow{2}{*} {$\mathcal{P}_{\rm ID}/\mathcal{\tilde{P}}_{\rm OOD}$}   &\multirow{2}{*} {Method}    &  \multicolumn{2}{c|}{Model Generalization}                                                    &\multicolumn{3}{c}{OOD Detection}                              \\
 &   &\text{Clean-Acc. $\uparrow$} & \text{Noise-Acc. $\uparrow$} & \text{FPR $\downarrow$}& \text{AUROC $\uparrow$}  &\text{AUPR $\uparrow$} \\ \midrule 
\multirow{3}{*} {\shortstack{ImageNet-200 / \\ \\None}}         &MSP        &  $\underline{85.15}^{\phantom{\pm0.01}}$   &  $74.84^{\phantom{\pm0.01}}$                                                  &$58.23^{\phantom{\pm0.01}}$  & $86.98^{\phantom{\pm0.01}}$  & $82.27^{\phantom{\pm0.01}}$                          \\  &Energy      &  $\underline{85.15}^{\phantom{\pm0.01}}$&  $74.84^{\phantom{\pm0.01}}$                                                  & $51.94^{\phantom{\pm0.01}}$ & $88.18^{\phantom{\pm0.01}}$   &$84.75^{\phantom{\pm0.01}}$                              \\ &Maxlogits      &  $\underline{85.15}^{\phantom{\pm0.01}}$&  $74.84^{\phantom{\pm0.01}}$                                                  & $\underline{51.62}^{\phantom{\pm0.01}}$ & $88.30^{\phantom{\pm0.01}}$   &$84.71^{\phantom{\pm0.01}}$                             \\\cline{1-7} \multirow{6}{*} {\shortstack{ImageNet-200 / \\ \\ImageNet-800}}  
    
     &Entropy      &   {${84.92}^{\phantom{\pm0.01}}$}    &${74.75}^{\phantom{\pm0.01}}$                                                    &\textcolor{mycolor4}{${53.62}^{\phantom{\pm0.01}}$}  &\textcolor{mycolor4}{$\underline{89.05}^{\phantom{\pm0.01}}$}   &\textcolor{mycolor4}{$\underline{85.02}^{\phantom{\pm0.01}}$}                              \\  
    
     &Energy      &   \textcolor{mycolor3}{$84.14^{\phantom{\pm0.01}}$}     &\textcolor{mycolor3}{$73.31^{\phantom{\pm0.01}}$}                                                    &\textcolor{mycolor3}{$59.73^{\phantom{\pm0.01}}$}  &\textcolor{mycolor4}{$87.54^{\phantom{\pm0.01}}$}     &\textcolor{mycolor4}{${82.81}^{\phantom{\pm0.01}}$}                                      \\  
    
     &DPN      &   $84.87^{\phantom{\pm0.01}}$     &$74.40^{\phantom{\pm0.01}}$                                                    &\textcolor{mycolor3}{$63.84^{\phantom{\pm0.01}}$}  &$87.18^{\phantom{\pm0.01}}$   &\textcolor{mycolor3}{$80.69^{\phantom{\pm0.01}}$}  \\  
    
     &Woods      &   ${84.99}^{\phantom{\pm0.01}}$     &$\underline{74.98}^{\phantom{\pm0.01}}$                                                    &\textcolor{mycolor4}{${51.71}^{\phantom{\pm0.01}}$}  &\textcolor{mycolor4}{$88.30^{\phantom{\pm0.01}}$}   &\textcolor{mycolor4}{${84.80}^{\phantom{\pm0.01}}$} \\ &SCONE      &  ${84.93}^{\phantom{\pm0.01}}$ &${74.91}^{\phantom{\pm0.01}}$                                                    &\textcolor{mycolor4}{${52.52}^{\phantom{\pm0.01}}$}  &\textcolor{mycolor4}{${88.19}^{\phantom{\pm0.01}}$}   &\textcolor{mycolor4}{${84.50}^{\phantom{\pm0.01}}$}                              \\
     &DUL (ours)      & \cellcolor{gray!20}\textcolor{mycolor4}{$\textbf{85.65}^{\pm0.07}$}  &\cellcolor{gray!20}\textcolor{mycolor4}{$\textbf{75.59}^{\pm0.12}$}                                                    &\cellcolor{gray!20}\textcolor{mycolor4}{$\textbf{49.14}^{\pm0.13}$}  &\cellcolor{gray!20}\textcolor{mycolor4}{$\textbf{89.27}^{\pm0.03}$}   &\cellcolor{gray!20}\textcolor{mycolor4}{$\textbf{85.62}^{\pm0.03}$}                              \\  
       \bottomrule
\end{tabular}}
\end{center}
\vskip -0.14in
\end{table*}




